Wireless Network Design Under Service Constraints

In this paper we consider the design of wireless queueing network control policies with special focus on application-dependent service constraints. In particular we consider streaming traffic induced requirements such as avoiding buffer underflows, which significantly complicate the control problem compared to guaranteeing throughput optimality only. Since state-of-the-art approaches for enforcing minimum buffer constraints in broadcast networks are not suitable for application in general networks we argue for a cost function based approach, which combines throughput optimality with flexibility regarding service constraints. New theoretical stability results are presented and various candidate cost functions are investigated concerning their suitability for use in wireless networks with streaming media traffic. Furthermore we show how the cost function based approach can be used to aid wireless network design with respect to important system parameters. The performance is demonstrated using numerical simulations.

==> figs/tandem.tex <==
% Graphic for TeX using PGF
% Title: /home/kasparick/Desktop/LATEX/draft-paper-allerton/gfx/tandem.dia
% Creator: Dia v0.97
% CreationDate: Wed May 30 12:20:34 2012
% For: kasparick
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{19.972668\du}{-61.147684\du}}
\pgfpathlineto{\pgfpoint{21.125168\du}{-61.147684\du}}
\pgfpathcurveto{\pgfpoint{21.443422\du}{-61.147684\du}}{\pgfpoint{21.701418\du}{-60.897833\du}}{\pgfpoint{21.701418\du}{-60.589626\du}}
\pgfpathcurveto{\pgfpoint{21.701418\du}{-60.281419\du}}{\pgfpoint{21.443422\du}{-60.031568\du}}{\pgfpoint{21.125168\du}{-60.031568\du}}
\pgfpathlineto{\pgfpoint{19.972668\du}{-60.031568\du}}
\pgfpathlineto{\pgfpoint{19.972668\du}{-61.147684\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{19.972668\du}{-61.147684\du}}
\pgfpathlineto{\pgfpoint{21.125168\du}{-61.147684\du}}
\pgfpathcurveto{\pgfpoint{21.443422\du}{-61.147684\du}}{\pgfpoint{21.701418\du}{-60.897833\du}}{\pgfpoint{21.701418\du}{-60.589626\du}}
\pgfpathcurveto{\pgfpoint{21.701418\du}{-60.281419\du}}{\pgfpoint{21.443422\du}{-60.031568\du}}{\pgfpoint{21.125168\du}{-60.031568\du}}
\pgfpathlineto{\pgfpoint{19.972668\du}{-60.031568\du}}
\pgfpathlineto{\pgfpoint{19.972668\du}{-61.147684\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (20.548918\du,-60.599626\du){$Q_1$};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{23.036710\du}{-61.170163\du}}
\pgfpathlineto{\pgfpoint{24.189210\du}{-61.170163\du}}
\pgfpathcurveto{\pgfpoint{24.507465\du}{-61.170163\du}}{\pgfpoint{24.765460\du}{-60.920312\du}}{\pgfpoint{24.765460\du}{-60.612105\du}}
\pgfpathcurveto{\pgfpoint{24.765460\du}{-60.303897\du}}{\pgfpoint{24.507465\du}{-60.054046\du}}{\pgfpoint{24.189210\du}{-60.054046\du}}
\pgfpathlineto{\pgfpoint{23.036710\du}{-60.054046\du}}
\pgfpathlineto{\pgfpoint{23.036710\du}{-61.170163\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{23.036710\du}{-61.170163\du}}
\pgfpathlineto{\pgfpoint{24.189210\du}{-61.170163\du}}
\pgfpathcurveto{\pgfpoint{24.507465\du}{-61.170163\du}}{\pgfpoint{24.765460\du}{-60.920312\du}}{\pgfpoint{24.765460\du}{-60.612105\du}}
\pgfpathcurveto{\pgfpoint{24.765460\du}{-60.303897\du}}{\pgfpoint{24.507465\du}{-60.054046\du}}{\pgfpoint{24.189210\du}{-60.054046\du}}
\pgfpathlineto{\pgfpoint{23.036710\du}{-60.054046\du}}
\pgfpathlineto{\pgfpoint{23.036710\du}{-61.170163\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (23.612960\du,-60.592105\du){$Q_2$};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.100000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{28.507949\du}{-61.171931\du}}
\pgfpathlineto{\pgfpoint{29.660449\du}{-61.171931\du}}
\pgfpathcurveto{\pgfpoint{29.978703\du}{-61.171931\du}}{\pgfpoint{30.236699\du}{-60.922080\du}}{\pgfpoint{30.236699\du}{-60.613872\du}}
\pgfpathcurveto{\pgfpoint{30.236699\du}{-60.305665\du}}{\pgfpoint{29.978703\du}{-60.055814\du}}{\pgfpoint{29.660449\du}{-60.055814\du}}
\pgfpathlineto{\pgfpoint{28.507949\du}{-60.055814\du}}
\pgfpathlineto{\pgfpoint{28.507949\du}{-61.171931\du}}
\pgfusepath{fill}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathmoveto{\pgfpoint{28.507949\du}{-61.171931\du}}
\pgfpathlineto{\pgfpoint{29.660449\du}{-61.171931\du}}
\pgfpathcurveto{\pgfpoint{29.978703\du}{-61.171931\du}}{\pgfpoint{30.236699\du}{-60.922080\du}}{\pgfpoint{30.236699\du}{-60.613872\du}}
\pgfpathcurveto{\pgfpoint{30.236699\du}{-60.305665\du}}{\pgfpoint{29.978703\du}{-60.055814\du}}{\pgfpoint{29.660449\du}{-60.055814\du}}
\pgfpathlineto{\pgfpoint{28.507949\du}{-60.055814\du}}
\pgfpathlineto{\pgfpoint{28.507949\du}{-61.171931\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (29.084199\du,-60.593872\du){$Q_m$};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetdash{{0.200000\du}{0.200000\du}}{0\du}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (18.317975\du,-60.599677\du)--(19.972668\du,-60.589626\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (21.750421\du,-60.596327\du)--(22.986585\du,-60.605396\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (24.765460\du,-60.612105\du)--(25.777951\du,-60.635032\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (27.634107\du,-60.635032\du)--(28.458232\du,-60.625000\du);
}
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetdash{{\pgflinewidth}{0.200000\du}}{0cm}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (26.202215\du,-60.635032\du)--(27.192165\du,-60.635032\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (20.837043\du,-60.589626\du){};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (17.367365\du,-60.592900\du){\large{$\alpha$}};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetdash{{0.200000\du}{0.200000\du}}{0\du}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (30.309543\du,-60.626052\du)--(31.964236\du,-60.616002\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (31.994945\du,-60.595222\du){$R_a$};
\end{tikzpicture}

